ObjectMover: Generative Object Movement with Video Prior

Simple as it seems, moving an object to another location within an image is, in fact, a challenging image-editing task that requires re-harmonizing the lighting, adjusting the pose based on perspective, accurately filling occluded regions, and ensuring coherent synchronization of shadows and reflections while maintaining the object identity. In this paper, we present ObjectMover, a generative model that can perform object movement in highly challenging scenes. Our key insight is that we model this task as a sequence-to-sequence problem and fine-tune a video generation model to leverage its knowledge of consistent object generation across video frames. We show that with this approach, our model is able to adjust to complex real-world scenarios, handling extreme lighting harmonization and object effect movement. As large-scale data for object movement are unavailable, we construct a data generation pipeline using a modern game engine to synthesize high-quality data pairs. We further propose a multi-task learning strategy that enables training on real-world video data to improve the model generalization. Through extensive experiments, we demonstrate that ObjectMover achieves outstanding results and adapts well to real-world scenarios.

==> table/insertion_metric.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\small % Reduce font size within the table
\begin{tabular}{l c c c c }
\toprule
\textbf{Method} & \textbf{PSNR} $\uparrow$ & \textbf{DINO-Score} $\uparrow$ & \textbf{CLIP-Score} $\uparrow$ & \textbf{DreamSim} $\downarrow$ \\
\midrule
Paint-by-Example~\cite{paint_by_example} & 20.83 & 53.87 & 81.98 & 0.457  \\
Anydoor~\cite{anydoor} & \underline{24.10} & \underline{77.49} & \underline{88.33} & \underline{0.223}  \\
Ours & \textbf{24.99} & \textbf{85.69} & \textbf{91.45} & \textbf{0.152}  \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitative comparisons on object insertion.} Our method consistently outperforms state-of-the-art methods.}
\label{tab:insertion}
\end{table}

